Looking for Confirmations: An Effective and Human-Like Visual Dialogue Strategy

Generating goal-oriented questions in Visual Dialogue tasks is a challenging and long-standing problem. State-Of-The-Art systems are shown to generate questions that, although grammatically correct, often lack an effective strategy and sound unnatural to humans. Inspired by the cognitive literature on information search and cross-situational word learning, we design Confirm-it, a model based on a beam search re-ranking algorithm that guides an effective goal-oriented strategy by asking questions that confirm the model's conjecture about the referent. We take the GuessWhat?! game as a case-study. We show that dialogues generated by Confirm-it are more natural and effective than beam search decoding without re-ranking.

==> introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

%Modelling task-oriented conversational agents is a long-standing and
%challenging problem. These systems have a wide range of potential
%applications in many different domains, and they are also suitable to
%study how artificial neural network architectures handle all the
%skills necessary to successfully accomplish the task at hand. In
%referential guessing games, in particular, two or more agents have to
%interact and cooperate to reach a goal, that is identifying a referent
%among a set of objects or symbolic data. 

Quite important progress has been made on multimodal conversational
systems thanks to the introduction of the Encoder-Decoder
framework~\cite{suts:seq14}. The success of these systems can be
measured by evaluating them on 
task-oriented referential games. Despite the high task-success reached
and the apparent linguistic
well-formedness of the single questions, the quality of the generated
dialogues, according to surface-level features, have been shown to be poor; this holds for systems based on both greedy and beam search~\cite{shekhar-etal-2019-beyond, zarriess-schlangen-2018-decoding, murahari-etal-2019-improving}.
\citet{test:inter2021} found that
when taking these surface-level features as a proxy of linguistic quality, the
latter does not correlate with task
success, and the authors point to the importance of studying deeper features
of dialogue structures. We aim to develop a multimodal model able to
generate more natural dialogues, namely
dialogues that resemble human dialogue strategies.  

Cognitive studies show that humans do not always act as ``rational''
agents. When referring to objects, they tend to be overspecific and prefer properties irrespectively of their utility for
identifying the referent~\cite{gatt2013bayesian};
% show that completely rational, utility-based accounts of reference production \cite{frank2012predicting} do not take into account the role of overspecification and preference rankings among properties that guide human speakers. 
when searching for information or when learning a language, they tend to follow
confirmation-driven strategies.  Modelling such behaviour in language learning,
\citet{medina2011words} and \citet{trueswell2013propose} propose 
%a win-stay,
%lose-shift one-trial 
a procedure in which a single hypothesized
word-referent pair is maintained across learning instances, and it is
abandoned only if the subsequent instance fails to confirm the
pairing, reflecting a `fast mapping' learning process. Inspired by
these theories, we propose a model, \textit{Confirm-it}, which
generates questions driven by the agent's confirmation bias.

%when searching for information orwhen learning word
%meaning they tend to follow confirmation-driven strategies.  

\begin{figure}[t]\centering
	\includegraphics[width=1\linewidth]{images/fig_intro_new_2.pdf}
	\caption{
		At turn 2, among the questions proposed by the beam
                search, \textit{Confirm-it}  chooses $b$  since it is the
                most suitable one to confirm the current conjecture.
		%An example of the dialogue strategy we discuss in the paper. Given a referential task, at turn 1 the agent formulates a conjecture about the referent given the dialogue history on top. At turn 2, the agent retrieves three hypotheses of the follow-up question using beam search, and it chooses the most suitable one to confirm its conjecture from the previous turn.
		%Example of the strategy followed by a human annotator playing the GuessWhat?!\cite{guesswhat_game} game as a Questioner. The target object the Oracle has in mind is marked in green. We conjecture that each question was uttered by having a specific candidate object in mind (see colour matching boxes).
		}
	\label{fig:intro}
	\vspace*{-6pt}
\end{figure}

Take the example of a
referential guessing game in which an agent has to ask questions to
guess an object in a given image. \textit{Confirm-it} will ask questions
that reinforce its beliefs about which is the target object, till
proven otherwise. For instance, in Figure~\ref{fig:intro}, after
learning that the target is a living entity (turn 1),  the agent conjectures
the target is the dog on the right of the picture (though in
principle, it could have been any of the candidates). Hence, the decoder generates the question that would let it confirm such
belief, ``is it a dog?''. If its expectations are not met (viz., it
receives a negative answer to such question -turn 2b), it moves its attention
to another candidate object.  
%which is most likely the target object and ask questions about it till
%evidences disconfirm its conjecture; at that point, it moves its
%attention to another candidate object and proceeds by looking for confirmations
%on that new single conjectured object. 
We do not claim that
our choice represents the optimal strategy to play the game,
but we believe that it makes the dialogue more natural in its flow
and  more effective because it takes into account the model's
intrinsic biases and intermediate predictions. 

%\at{(Avevamo deciso di fare riferimento qualche riga sopra alla figura 1, ma allora non posso mettere "Confirm-it" nella caption. Altrimenti mettiamo "single-conjecture strategy" nella caption.)}

%We take the GuessWhat?!\@ referential visual guessing
%game \cite{guesswhat_game} as a test-bed for our experiments. In
%GuessWhat?!\@, an Oracle is assigned a target object in a visual scene, and
%a Questioner asks polar questions to an Oracle in
%order to identify the target  \rb{(see Figure \ref{fig:intro})}.  A
%manual inspections of the human dialogues reveals that GuessWhat?!
%players tend to use this confirmation-driven strategy to a large
%degree.  \rb{For instance, the GuessWhat?!\@ player of the game illustrated in Figure~\ref{fig:intro} starts by implicitly formulating a hypothesis about the target. The player conjectures that the red ribbon is the target, and he/she asks questions to verify this supposition. The answer to the second question, however, proves that the Questioner was wrong; a new hypothesis is formulated (the white object) and immediately disproved by the Oracle. The Questioner then conjectures that the scissors on the left are the target object, obtaining a confirmation to his/her question at the fourth turn and a denial at the final question, when the target becomes clear.}


 
%is the core
%architecture of most current task-oriented multimodal
%conversational systems.

% A simple but efficient implementation of the
%decoder is based on greedy search which generates the most likely word
%at each time step at the risk of generating low-quality
%dialogues. Alternative common approaches let the model
%generate a fixed number of alternative hypotheses through beam search, and use som%e further
%criterion to prune or re-rank such alternatives~\cite{}. \at{La parte
 % che precede su greedy/beam la discutiamo anche nei related. In
 % questo punto mi sembra un po' slegata dal contesto.}

%The importance of considering both task success and dialogue quality has
%been advocated in~\cite{shekhar-etal-2019-beyond} who compared
%generated dialogues based on surface-level features, such as
%repetitions and vocabulary richness.  

%When
%considering multimodal tasks, one striking feature of the generated
%dialogues that could explain the observations in
%\citet{test:inter2021} is the lack of an effective strategy to
%identify a referent in complex and naturalistic visual scenes,
%plausibly due to an over-reliance on language priors.




%The question
%generator and the guesser modules are trained jointly in an
%end-to-end fashion.  
%It is thus clear that following
%a strategy while asking questions is a key ingredient to accomplish
%this task. 
\cut{\citet{mazuecos-etal-2020-role} compared GDSE against other State-Of-The-Art
models playing the Questioner task by measuring the
\textit{effectiveness} of each question, defined as the ability of a
question to discard candidate objects in the visual scene that are not
the target. The authors found that, for the majority of the models
considered, successful dialogues do not have a higher percentage of
effective questions based on this metric, and that the
model closest to humans is VDST~\cite{pang_gw}.
%, whose question generator model is based on a visual dialogue state tracking (VDST)~\cite{}. 
VDST uses the probability distribution of the guesser to guide the question
 generator, and it builds on the assumption that at turn zero all objects are equally
  probable. We diverge from this assumption but we agree on the
importance of establishing a tied connection between the probability
distribution assigned by the Guesser to the candidate objects and the
generation of questions. \at{Forse questo paragrafo si può accorciare parecchio.}
}

To evaluate this strategy, we take as a test-bed GuessWhat?!\@
\cite{guesswhat_game}, a two-player game between a Questioner that has to guess the target and an Oracle.  
%We develop \textit{Confirm-it}, a new model of the Questioner agent that is able to perform all the three tasks involved: asking question (QGen), guessing the target (Guesser), and answering questions (Oracle).
The widely used architecture of the Questioner, GDSE, jointly train a Question Generator (QGen) and a Guesser~\cite{shekhar-etal-2019-beyond}.  We  augment it with a module that simulates an internal oracle. 
The three modules of the Questioner straightly cooperate one
with the other: the internal oracle guides the question generator to
ask questions that reinforce the Guesser's beliefs. Concretely, at
training time, through Supervised Learning (SL) the QGen
learns to ask human-like questions turn-by-turn, the internal oracle
to answer them, and the guesser to guess the target
object once the dialogue ends. At test time, we exploit a beam search re-ranking
algorithm that simulates the single-conjecture learning strategy used
by humans. Among the questions the QGen 
generates via beam search, the algorithm promotes the one that helps the guesser
reinforce its belief.
% At each dialogue
%turn, based on the multimdal representation of the dialogue history,
%the guesser module formulates a prediction about the target object,
%while \textit{} promotes the generation of questions that look for
%evidence to confirm the model's conjecture about the
%target. \textit{PbV-ReRank} asks its internal Oracle model to answer
%each question retrieved by the beam search as if the model's
%conjecture was indeed the target object. \textit{PbV-ReRank} selects
%the question that is more suitable to confirm its hypothesis about the
%target. 

We run both quantitative and qualitative analyses, and evaluate the
effectiveness of the dialogue strategy by asking humans to guess the
target given dialogues generated by \textit{Confirm-it}. We compare
results when giving the dialogue generated by \textit{Confirm-it}
using the re-ranking algorithm and when generating the question
proposed by the plain beam search. We show
that the task accuracy both of 
the conversational agent and human subjects increases when receiving
dialogues generated by the \textit{Confirm-it} re-ranking. 
%\rb{the
 % other metrics..} \at{Serve parlare delle altre metriche? Forse basta quello scritto all'inizio del paragrafo}

%compared  the plain beam search decoding. 
%Hence, without the need for any further
%training or additional parameters compared to the model trained in a
%Supervised Learning fashion.

%\at{(a) La figura 1 mi sembra un po' "vuota" come immagine (tanto spazio bianco, poche informazioni rispetto a quello che troviamo nella introduzione). (b) Non diciamo in nessun punto che la strategia che vogliamo implementare è stata osservata anche nei dialoghi umani.}

%\rb{We show that this re-ranking strategy improves the accuracy in
%the GuessWhat?!\@ guessing game by around 5\%, without the need for
%any further training nor additional parameters compared to the model
%trained in a Supervised Learning fashion.} 

